On the Benefits of Multiple Gossip Steps in Communication-Constrained Decentralized Optimization

In decentralized optimization, it is common algorithmic practice to have nodes interleave (local) gradient descent iterations with gossip (i.e. averaging over the network) steps. Motivated by the training of large-scale machine learning models, it is also increasingly common to require that messages be {\em lossy compressed} versions of the local parameters. In this paper, we show that, in such compressed decentralized optimization settings, there are benefits to having {\em multiple} gossip steps between subsequent gradient iterations, even when the cost of doing so is appropriately accounted for e.g. by means of reducing the precision of compressed information. In particular, we show that having $O(\log\frac{1}{\epsilon})$ gradient iterations {with constant step size} - and $O(\log\frac{1}{\epsilon})$ gossip steps between every pair of these iterations - enables convergence to within $\epsilon$ of the optimal value for smooth non-convex objectives satisfying Polyak-\L{}ojasiewicz condition. This result also holds for smooth strongly convex objectives. To our knowledge, this is the first work that derives convergence results for nonconvex optimization under arbitrary communication compression.

==> aistats_experiments.tex <==
%%%% Figure 1 
%%%% Plot Effect of Q in compensating information Loss induced by lower consensus lr
%%% --------------------------------------------------
%%%% Figure -2 
%%%% Plot Effect of Topology for different n_cores
%%%%% ------------------------------------------------
%% Figure-3 
%% Compare Compression Schemes 
%%%%%%%%%%%%%%%%%%%%%%%%
We verify our theory on three simple yet common machine learning problems - logistic regression, linear regression and non-linear regression. %\footnote{We show the results of effect of varying $Q$ and varying network topologies for all three datasets here. Since the results of $\mathrm{rand}({\omega})$ and $\mathrm{rand2}({\omega})$ were nearly identical, we only show the plots for $\mathrm{rand}({\omega})$.}
{\color{black} Due to lack of space, we defer the experiments on logistic regression on MNIST to the supplementary material where we further explore various network topologies and compression schemes.}
%Following \cite{koloskova2019decentralized}, for all the experiments we plot the sub-optimality, i.e. $f(\bar{\x}_{t}) - f^\ast$ against the number of local gradient computations (or steps).
%Here, $f^\ast$ is the optimal value obtained by running vanilla gradient descent with the entire data on a single machine -- we shall refer to this setting as "Centralized GD" throughout this section. 
{\color{black} We consider the top($k$) and $\textrm{qsgd}$ compression schemes and %consider 
the torus topology to represent the communication graph of the network (see, e.g. \cite{xiao2004fast,koloskova2019decentralized}). %All plots are averaged over 3 independent runs
}Before describing our experimental set-up, we describe the datasets.
%\subsection{Datasets} 

Let $\{s^{(i)}_{1},\ldots,s^{(i)}_{n_{i}}\}$ denote the samples being processed in the $i\ts{th}$ node where $n_{i}$ is the total number of samples in the $i\ts{th}$ node.
Then, $f_{i}(\x) = \frac{1}{n_{i}} \sum_{j=1}^{n_{i}} \ell (\x,s^{(i)}_{j})$, where $\ell(.)$ denotes the loss function of the regression tasks that we explain next.

% {
% \color{blue}
% %\subsubsection{Logistic regression} 
% \textit{Logistic Regression:}
% We use a binary version of MNIST \cite{lecun1998gradient} where the first five classes are treated as class 0 and the rest as class 1. We train a classifier with the binary cross-entropy loss. 
% We consider a decentralized setting where the data is evenly distributed among all the nodes in a challenging sorted setting (sorted based on labels) where at most one node  acquires examples from both classes. 
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Linear regression} 
\textit{Linear Regression:}
We train a linear regression model on $m=10000$ synthetic data samples $\{(\mathbf{a}_{i},y_{i})\}_{i=1}^{m}$ generated according to $y_{i} = \langle \boldsymbol{\theta}^\ast, \mathbf{a}_{i} \rangle + e_{i}$, where $\boldsymbol{\theta}^\ast \in \mathbb{R}^{2000}$, the $i\ts{th}$ input $\mathbf{a}_{i} \sim \mathcal{N}(\mathbf{{0}}, I_{2000})$, and noise $e_{i} \sim \mathcal{N}(0,0.05)$. We refer to this %synthetic 
dataset as SYN-1. Here, we use the squared loss function with $\ell_{2}$-regularization.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{Non-convex non-linear regression} 
\textit{Non-Convex Non-Linear Regression:}
We train a non-linear regression model on $m=10000$ synthetic data samples $\{(\mathbf{a}_{i},y_{i})\}_{i=1}^{m}$ generated as $y_i = \text{relu}(\langle \boldsymbol{\theta}^\ast, \mathbf{a}_i \rangle) + e_i$, where $\boldsymbol{\theta}^\ast \in \mathbb{R}^{2000}$, the $i\ts{th}$ input $\mathbf{a}_i \sim \mathcal{N}(\vec{{0}}, I_{2000})$, $e_i \sim \mathcal{N}(0,0.05)$ and $\text{relu}(z) = \text{max}(z,0)$ (i.e. the standard ReLU function). 
We call this synthetic dataset SYN-2 henceforth. We model this task as training a one-layer neural network having ReLU activation with the squared loss function and {$\ell_{2}$-regularization.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{
\color{black}
%\subsection{Experimental Setting: Fixed Communication Budget Per Iteration}
\textbf{Experimental Setting -- Fixed Communication Budget Per Iteration.}
In order to illustrate the value of having more gossiping steps (i.e. larger $Q$), we consider a simple setting where our communication budget in every iteration (involving one gradient computation step and $Q$ gossiping steps) is fixed. So for top-$k$/rand-$k$, we keep $Q k$ constant, whereas for $b$-bit qsgd, $Q b$ is kept constant. Since $Q k$/$Q b$ is kept constant, the total number of bits communicated will be proportional to the number of iterations $T$ (which is the  horizontal axis of the plots in Figures \ref{fig:1} and \ref{fig:2}).
%\\
In \Cref{fig:1}, we plot the training loss on the vertical axis (in log-scale) vs. the number of bits (order wise) on the horizontal axis for SYN-2 (non-convex non-linear regression) with qsgd. We maintain $Qb = 8$ and consider 3 different consensus learning rates $\gamma = \{0.05,0.1,0.15\}$ (keeping everything else the same).
%\\

In \Cref{fig:2}, we show similar plots for SYN-1 (strongly convex linear regression task) with top-$k$. Let $\omega = (k/d)*100$ ($d$ being the dimension of the vectors). We keep $Q\omega = 100$ (note that this is the same as maintaining $Q k$ constant) and consider 3 different values of the number of nodes $n = \{9,16,25\}$ (keeping everything else the same).
%\\
% {All plots are averaged over 3 independent runs where we consider the torus topology to represent the communication graph of the network.}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Significance of large Q} 
\textbf{Significance of large Q.}
In both \Cref{fig:1} and \Cref{fig:2}, observe that higher $Q$ at the expense of more aggressive compression leads to fewer gross total number of bits communicated -- as predicted by the results established in the beginning of  Section \ref{sec:dissc}. Note that if latency/synchronization time between the nodes is negligible, then having higher $Q$ also leads to faster convergence (since the total number of bits is proportional to $T$ in our setting). Further, in \Cref{fig:2} (for SYN-1, which has a strongly convex objective), observe that higher $Q$ results in almost straight line curves (recall that the training loss is plotted in log-scale) -- implying linear convergence. Further note that for $Q=1$ the curves are not straight lines. This verifies our theoretical findings in Corollary \ref{cor:1}. 
%The backbone of DeLi-CoCo is the introduction of performing $Q$ mixing steps. To better understand the role of this stage under communication compression, in \Cref{fig:Q} we depict the performance of DeLi-CoCo for different values of $Q$ under varied consensus learning rates $\gamma$ where we compare its performance to centralized GD without compression.  Our experiments suggest that DeLi-CoCo can achieve the same rate of convergence as Centralized GD for suitable values of $Q$, thereby illustrating the value of having multiple mixing steps. We further observe that with higher $\gamma$, DeLi-CoCo requires fewer mixing steps to match the performance of Centralized GD. 
%%%%%%% TOPOLOGY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Supplementary Material}
\begin{comment}
\subsection{Impact of Topology}
\Cref{fig:T} shows the effect of  topology and size of the network on the convergence of DeLi-CoCo under communication compression. 
We repeatedly observe that fully connected topology outperforms torus which is followed by the ring topology, consistent with the intuition that better connectivity leads to faster convergence. %We further show 
Notice that increasing the number of nodes worsens the convergence across all topologies. However, this effect is less severe for the networks with stronger connectivity properties. This observation is consistent with the intuition that communication compression leads to weakening of network connectivity.
Also note that increasing $Q$ improves the rate of convergence, reinforcing our earlier observations in \Cref{fig:Q}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impact of Compression Operator}
In \Cref{fig:C}, we show the effect of different compression schemes on the rate of convergence. In particular, we compare DeLi-CoCo with the DGD \cite{nedic2009distributed,yuan2016convergence} that operates under no communication compression (i.e., full communication). %with $\gamma=1$ and $Q=1$. 
Note that with majority of the compression schemes, DeLi-CoCo achieves similar rates as DGD.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Discussion: Fixed Communication Budget}
% As we discussed, our main idea in this paper is that given a \textit{fixed communication budget per iteration}, having multiple gossip steps with aggressive
% compression is preferred to having just one gossip step with higher precision communication. To illustrate this in an
% experiment, we consider SYN-2 settings where $Q \times \omega$ is constant ($\omega$ is proportional to the amount of information transmitted).
% In Figure~4, we compare our method with Choco-GD (deterministic variant of \cite{koloskova2019decentralized}) and use QSGD for quantization. 
% Notice that the amount of communicated bits per gradient computation is identical for all schemes in Figure~4. This shows that our approach uses significantly
% fewer bits to achieve a target 
% sub-optimality level ($f-f^{*}$) of $\epsilon = 0.01$. Further, given the considerable performance gap in Figure~4, our approach would be preferable even after accounting for a reasonable level of latency/overhead.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%   \begin{center}
%     \includegraphics[width=0.5\textwidth]{../experiments/fig44.png}
%   \end{center}
%   \caption{\footnotesize Comparison of the proposed scheme and the benchmark \cite{koloskova2019decentralized} on the non-convex task described by SYN-2 given a fixed communication budget per iteration.}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 






 






==> experiment.tex <==
%%%% Figure 1 
%%%% Plot Effect of Q in compensating information Loss induced by lower consensus lr
%%% --------------------------------------------------
\begin{figure}[!htb]
\centering
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/results_mnist_partial/Q_0.1.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/results_mnist_partial/Q_0.5.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/results_mnist_partial/Q_1.0.eps}} \\

\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN1-figs/fig1_0.05.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN1-figs/fig1_0.1.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN1-figs/fig1_0.2.eps}} 

\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN2-figs/fig1_0.05.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN2-figs/fig1_0.1.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN2-figs/fig1_0.15.eps}} 
\caption{\small Effect of varying $Q$ under different consensus learning rates $\gamma$.   MNIST setting (top row): $n=9$, $\mathrm{top}({0.05})$; SYN-1 setting (mid row): $n=16$, $\mathrm{qsgd}_{2}$; SYN-2 (bottom row): $n=16$, $\mathrm{qsgd}_{2}$, $\ell_2$-regularization value = 0.001. We used $\eta = 0.2$ and torus topology for all datasets.
}
\label{fig:Q}
\end{figure} 
%%%% Figure -2 
%%%% Plot Effect of Topology for different n_cores
%%%%% ------------------------------------------------
\begin{figure}[!htb]
\centering
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/results_mnist_partial/T_9.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/results_mnist_partial/T_16.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/results_mnist_partial/T_25.eps}}

\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN1-figs/fig2_9.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN1-figs/fig2_16.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN1-figs/fig2_25.eps}}

\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN2-figs/fig2_9.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN2-figs/fig2_16.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{../experiments/new-SYN2-figs/fig2_25.eps}} 
\caption{\small Effect of network topology settings on the convergence rates; showing dependence on the number of nodes $n$ and mixing steps $Q$. MNIST setting(top row): $\mathrm{top}({0.05})$, $\gamma = 0.5$, $\eta=0.2$. SYN-1 setting (bottom row): $\mathrm{qsgd}_{2}$, $\gamma = 0.1$; We used $\eta=0.2$ for $n=9,16$ and $\eta=0.15$ for $n=25$, respectively.
SYN2 setting (bottom row): $\mathrm{qsgd}_{2}$, $\eta=0.2$, $\ell_2$-regularization parameter = 0.001; We used $\gamma = 0.1$ for $n=9, 16$ and $\gamma = 0.15$ for $n=25$.
}
\label{fig:T}
\end{figure}
%% Figure-3 
%% Compare Compression Schemes 
\begin{figure}[t]
\centering 
\subfloat{\includegraphics[width=0.33\textwidth]{experiments/results_mnist_partial/C.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{experiments/new-SYN1-figs/fig3.eps}}
\subfloat{\includegraphics[width=0.33\textwidth]{experiments/new-SYN2-figs/fig3.eps}}
\caption{\footnotesize Comparison of various compression operators over torus topology. MNIST (Left): $n=9, \eta = 0.2$; For $\mathrm{qsgd}_{2}$, $\mathrm{top}(0.05)$, $\mathrm{rand}(0.05)$, we used $Q = \{10,15,15\}$ and $\gamma =\{0.05,0.1,0.05\}$, respectively. SYN-1 (Middle): $n=16, \eta = 0.2$, $Q=5$;
For $\mathrm{qsgd}_{2}$, $\mathrm{top}(0.05)$, and $\mathrm{rand}(0.05)$, we used $\gamma = 0.2$, $0.2$ and $ 0.05$, respectively. SYN2 (Right): $n=16, \eta = 0.2$, $Q=5$, $\ell_2$-regularization parameter = 0.001; For $\mathrm{qsgd}_{2}$, $\mathrm{top}(0.05)$, and $\mathrm{rand}(0.05)$ we used $\gamma = 0.2$, $\gamma = 0.2$, and $\gamma = 0.05$, respectively.}
\label{fig:C}
\vspace{-3mm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%
We verify our theory on three common machine learning problems - logistic regression, linear regression and non-linear regression.\footnote{We show the results of effect of varying $Q$ and varying network topologies for all three datasets here. Since the results of $\mathrm{rand}({\omega})$ and $\mathrm{rand2}({\omega})$ were nearly identical, we only show the plots for $\mathrm{rand}({\omega})$.} Following \cite{koloskova2019decentralized}, for all the experiments we plot the sub-optimality, i.e. $f(\bar{\x}_{t}) - f^\ast$ against the number of local gradient computations (or steps). Here, $f^\ast$ is the optimal value obtained by running vanilla gradient descent with the entire data on a single machine -- we shall refer to this setting as "Centralized GD" throughout this section. We consider the compression schemes proceeding the statement of Assumption 4, and explore some network topologies commonly used in literature, namely ring, torus, fully-connected and disconnected topologies (see, e.g. \cite{xiao2004fast,koloskova2019decentralized}). 
All plots are averaged over 3 independent runs.

\subsection{Datasets} 
Let $\{s^{(i)}_{1},\ldots,s^{(i)}_{n_{i}}\}$ denote the samples being processed in the $i\ts{th}$ node where $n_{i}$ is the total number of samples in the $i\ts{th}$ node.
Then, $f_{i}(\x) = \frac{1}{n_{i}} \sum_{j=1}^{n_{i}} \ell (\x,s^{(i)}_{j})$, where $\ell(.)$ denotes the loss function of the regression tasks that we explain next.

\subsubsection{Logistic regression} 
We use a binary version of MNIST \cite{lecun1998gradient} where the first five classes are treated as class 0 and the rest as class 1. We train a classifier with the binary cross-entropy loss. 
We consider a decentralized setting where the data is evenly distributed among all the nodes in a challenging sorted setting (sorted based on labels) where at most one node  acquires examples from both classes. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear regression} 
We train a linear regression model on $m=10000$ synthetic data samples $\{(\mathbf{a}_{i},y_{i})\}_{i=1}^{m}$ generated according to $y_{i} = \langle \boldsymbol{\theta}^\ast, \mathbf{a}_{i} \rangle + e_{i}$, where $\boldsymbol{\theta}^\ast \in \mathbb{R}^{2000}$, the $i\ts{th}$ input $\mathbf{a}_{i} \sim \mathcal{N}(\mathbf{{0}}, I_{2000})$, and noise $e_{i} \sim \mathcal{N}(0,0.05)$. We refer to this synthetic dataset as SYN-1. Here, we use the squared loss function with $\ell_{2}$-regularization value = 0.001.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Non-convex non-linear regression} 
We train a non-linear regression model on $m=10000$ synthetic data samples $\{(\mathbf{a}_{i},y_{i})\}_{i=1}^{m}$ generated as $y_i = \text{relu}(\langle \boldsymbol{\theta}^\ast, \mathbf{a}_i \rangle) + e_i$, where $\boldsymbol{\theta}^\ast \in \mathbb{R}^{2000}$, the $i\ts{th}$ input $\mathbf{a}_i \sim \mathcal{N}(\vec{{0}}, I_{2000})$, $e_i \sim \mathcal{N}(0,0.05)$ and $\text{relu}(z) = \text{max}(z,0)$ (i.e. the standard ReLU function). 
We call this synthetic dataset SYN-2 henceforth. We model this task as training a one-layer neural network having ReLU activation with the squared loss function and {$\ell_{2}$-regularization value = 0.001}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Importance of Q} 
The backbone of DeLi-CoCo is the introduction of performing $Q$ mixing steps. To better understand the role of this stage under communication compression, in \Cref{fig:Q} we depict the performance of DeLi-CoCo for different values of $Q$ under varied consensus learning rates $\gamma$ where we compare its performance to centralized GD without compression.  Our experiments suggest that DeLi-CoCo can achieve the same rate of convergence as Centralized GD for suitable values of $Q$, thereby illustrating the value of having multiple mixing steps. We further observe that with higher $\gamma$, DeLi-CoCo requires fewer mixing steps to match the performance of Centralized GD. 
%%%%%%% TOPOLOGY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impact of Topology}
\Cref{fig:T} shows the effect of  topology and size of the network on the convergence of DeLi-CoCo under communication compression. 
We repeatedly observe that fully connected topology outperforms torus which is followed by the ring topology, consistent with the intuition that better connectivity leads to faster convergence. %We further show 
Notice that increasing the number of nodes worsens the convergence across all topologies. However, this effect is less severe for the networks with stronger connectivity properties. This observation is consistent with the intuition that communication compression leads to weakening of network connectivity.
Also note that increasing $Q$ improves the rate of convergence, reinforcing our earlier observations in \Cref{fig:Q}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Impact of Compression Operator}
In \Cref{fig:C}, we show the effect of different compression schemes on the rate of convergence. In particular, we compare DeLi-CoCo with the DGD \cite{nedic2009distributed,yuan2016convergence} that operates under no communication compression (i.e., full communication). %with $\gamma=1$ and $Q=1$. 
Note that with majority of the compression schemes, DeLi-CoCo achieves similar rates as DGD.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussion: Fixed Communication Budget}
% As we discussed, our main idea in this paper is that given a \textit{fixed communication budget per iteration}, having multiple gossip steps with aggressive
% compression is preferred to having just one gossip step with higher precision communication. To illustrate this in an
% experiment, we consider SYN-2 settings where $Q \times \omega$ is constant ($\omega$ is proportional to the amount of information transmitted).
% In Figure~4, we compare our method with Choco-GD (deterministic variant of \cite{koloskova2019decentralized}) and use QSGD for quantization. 
% Notice that the amount of communicated bits per gradient computation is identical for all schemes in Figure~4. This shows that our approach uses significantly
% fewer bits to achieve a target 
% sub-optimality level ($f-f^{*}$) of $\epsilon = 0.01$. Further, given the considerable performance gap in Figure~4, our approach would be preferable even after accounting for a reasonable level of latency/overhead.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%   \begin{center}
%     \includegraphics[width=0.5\textwidth]{../experiments/fig44.png}
%   \end{center}
%   \caption{\footnotesize Comparison of the proposed scheme and the benchmark \cite{koloskova2019decentralized} on the non-convex task described by SYN-2 given a fixed communication budget per iteration.}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 






 





